Trapped Modes and Steered Dirac Cones in Platonic Crystals

This paper discusses the properties of flexural waves obeying the biharmonic equation, propagating in a thin plate pinned at doubly-periodic sets of points. The emphases are on the properties of dispersion surfaces having the Dirac cone topology, and on the related topic of trapped modes in plates with a finite set (cluster) of pinned points. The Dirac cone topologies we exhibit have at least two cones touching at a point in the reciprocal lattice, augmented by another band passing through the point. We show that the Dirac cones can be steered along symmetry lines in the Brillouin zone by varying the aspect ratio of rectangular lattices of pins, and that, as the cones are moved, the involved band surfaces tilt. We link Dirac points with a parabolic profile in their neighbourhood, and the characteristic of this parabolic profile decides the direction of propagation of the trapped mode in finite clusters.

==> macro.tex <==
% Reduce space surrounding equal signs (=) in equation arrays.
\setlength{\arraycolsep}{2pt}
% Set up counter for list environments
\newcounter{itemnbr}
% Handy abbreviations.
\newcommand\eq[1] {(\ref{#1})}
\newcommand\eqp[1] {(\ref{eq:#1})}
\newcommand\defn[1] {\ref{def:#1}}
\newcommand\thm[1] {\ref{thm:#1}}
\newcommand\sect[1] {\ref{sec:#1}}
\newcommand\fig[1] {\ref{fig:#1}}
\newcommand\labeq[1] {\label{eq:#1}}
\newcommand\labdefn[1] {\label{def:#1}}
\newcommand\labthm[1] {\label{thm:#1}}
\newcommand\labsect[1] {\label{sec:#1}}
\newcommand\labfig[1] {\label{fig:#1}}
\newcommand\etal{{\it et al.}}
%\newcommand\B {\Bigg}
% Math environments
\newtheorem{definition}{Definition}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
%\newcommand\proof{{\it Proof:}\quad}
\newcommand\remark{{\it Remark:}\quad}
%\newcommand\qed{\ \rule[-0.2ex]{0.3em}{1.5ex}}
% De-verbose the LaTeX math environment
\newcommand{\bfm}[1]{\mbox{\boldmath ${#1}$}}
\newcommand{\nonum}{\nonumber \\}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}[1]{\label{#1}\end{eqnarray}}
\newcommand{\bequ}{\begin{equation}}
\newcommand{\eequ}[1]{\label{#1}\end{equation}}
%\newcommand{\R}{\mbox{R}}
%\newcommand{\C}{\mbox{C}}
\newcommand{\Grad}{\nabla}
%\newcommand{\Div}{\nabla \cdot}
\newcommand{\Curl}{\nabla \times}
\newcommand{\mn}{{\rm min}}
\newcommand{\mx}{{\rm max}}
\newcommand{\lang}{\langle}
\newcommand{\rang}{\rangle}
\newcommand{\Md}{\partial}
\newcommand{\MP}{\bigoplus}
\newcommand{\MT}{\bigotimes}
\newcommand{\MU}{\bigcup}
\newcommand{\MI}{\bigcap}
\newcommand{\MV}{\bigvee}
\newcommand{\MW}{\bigwedge}
\newcommand{\ov}[1]{\overline{#1}}

% Abbreviate definitions of greek symbols
\newcommand{\Ga}{\alpha}
\newcommand{\Gb}{\beta}
\newcommand{\Gd}{\delta}
\newcommand{\Ge}{\epsilon}
\newcommand{\Gve}{\varepsilon}
\newcommand{\Gf}{\phi}
\newcommand{\Gvf}{\varphi}
\newcommand{\Gg}{\gamma}
\newcommand{\Gc}{\chi}
\newcommand{\Gi}{\iota}
\newcommand{\Gk}{\kappa}
\newcommand{\Gl}{\lambda}
\newcommand{\Gn}{\eta}
\newcommand{\Gm}{\mu}
\newcommand{\Gv}{\nu}
\newcommand{\Gp}{\pi}
\newcommand{\Gt}{\theta}
\newcommand{\Gvt}{\vartheta}
\newcommand{\Gr}{\rho}
\newcommand{\Gvr}{\varrho}
\newcommand{\Gs}{\sigma}
\newcommand{\Gvs}{\varsigma}
\newcommand{\Gj}{\tau}
\newcommand{\Gu}{\upsilon}
\newcommand{\Go}{\omega}
\newcommand{\Gx}{\xi}
\newcommand{\Gy}{\psi}
\newcommand{\Gz}{\zeta}
\newcommand{\GD}{\Delta}
\newcommand{\GF}{\Phi}
%\newcommand{\GG}{\Gamma}
\newcommand{\GL}{\Lambda}
\newcommand{\GP}{\Pi}
\newcommand{\GT}{\Theta}
\newcommand{\GS}{\Sigma}
\newcommand{\GU}{\Upsilon}
\newcommand{\GO}{\Omega}
\newcommand{\GX}{\Xi}
\newcommand{\GY}{\Psi}

% Abbreviate definitions of bold greek symbols: note that defs.tex is 
% needed first
\newcommand{\BGa}{\bfm\alpha}
\newcommand{\BGb}{\bfm\beta}
\newcommand{\BGd}{\bfm\delta}
\newcommand{\BGe}{\bfm\epsilon}
\newcommand{\BGve}{\bfm\varepsilon}
\newcommand{\BGf}{\bfm\phi}
\newcommand{\BGvf}{\bfm\varphi}
\newcommand{\BGg}{\bfm\gamma}
\newcommand{\BGc}{\bfm\chi}
\newcommand{\BGi}{\bfm\iota}
\newcommand{\BGk}{\bfm\kappa}
\newcommand{\BGl}{\bfm\lambda}
\newcommand{\BGn}{\bfm\eta}
\newcommand{\BGm}{\bfm\mu}
\newcommand{\BGv}{\bfm\nu}
\newcommand{\BGp}{\bfm\pi}
\newcommand{\BGt}{\bfm\theta}
\newcommand{\BGvt}{\bfm\vartheta}
\newcommand{\BGr}{\bfm\rho}
\newcommand{\BGvr}{\bfm\varrho}
\newcommand{\BGs}{\bfm\sigma}
\newcommand{\BGvs}{\bfm\varsigma}
\newcommand{\BGj}{\bfm\tau}
\newcommand{\BGu}{\bfm\upsilon}
\newcommand{\BGo}{\bfm\omega}
\newcommand{\BGx}{\bfm\xi}
\newcommand{\BMx}{\bfm\xi}
\newcommand{\BGy}{\bfm\psi}
\newcommand{\BGz}{\bfm\zeta}
\newcommand{\BGD}{\bfm\Delta}
\newcommand{\BGF}{\bfm\Phi}
\newcommand{\BGG}{\bfm\Gamma}
\newcommand{\BGL}{\bfm\Lambda}
\newcommand{\BGP}{\bfm\Pi}
\newcommand{\BGT}{\bfm\Theta}
\newcommand{\BGS}{\bfm\Sigma}
\newcommand{\BGU}{\bfm\Upsilon}
\newcommand{\BGO}{\bfm\Omega}
\newcommand{\BGX}{\bfm\Xi}
\newcommand{\BGY}{\bfm\Psi}


% Abbreviate symbols for caligraphic letters
\newcommand{\Ca}{{\cal a}}
\newcommand{\Cb}{{\cal b}}
\newcommand{\Cc}{{\cal c}}
\newcommand{\Cd}{{\cal d}}
\newcommand{\Ce}{{\cal e}}
\newcommand{\Cf}{{\cal f}}
\newcommand{\Cg}{{\cal g}}
\newcommand{\Ch}{{\cal h}}
\newcommand{\Ci}{{\cal i}}
\newcommand{\Cj}{{\cal j}}
\newcommand{\Ck}{{\cal k}}
\newcommand{\Cl}{{\cal l}}
\newcommand{\Cm}{{\cal m}}
\newcommand{\Cn}{{\cal n}}
\newcommand{\Co}{{\cal o}}
\newcommand{\Cp}{{\cal p}}
\newcommand{\Cq}{{\cal q}}
\newcommand{\Cr}{{\cal r}}
\newcommand{\Cs}{{\cal s}}
\newcommand{\Ct}{{\cal t}}
\newcommand{\Cu}{{\cal u}}
\newcommand{\Cv}{{\cal v}}
\newcommand{\Cx}{{\cal x}}
\newcommand{\Cy}{{\cal y}}
\newcommand{\Cz}{{\cal z}}
\newcommand{\CA}{{\cal A}}
\newcommand{\CB}{{\cal B}}
%\newcommand{\CC}{{\cal C}}
%\newcommand{\CD}{{\cal D}}
\newcommand{\CE}{{\cal E}}
\newcommand{\CF}{{\cal F}}
%\newcommand{\CG}{{\cal G}}
\newcommand{\CH}{{\cal H}}
\newcommand{\CI}{{\cal I}}
\newcommand{\CJ}{{\cal J}}
\newcommand{\CK}{{\cal K}}
\newcommand{\CL}{{\cal L}}
\newcommand{\CM}{{\cal M}}
\newcommand{\CN}{{\cal N}}
\newcommand{\CO}{{\cal O}}
\newcommand{\CP}{{\cal P}}
\newcommand{\CQ}{{\cal Q}}
\newcommand{\CR}{{\cal R}}
\newcommand{\CS}{{\cal S}}
\newcommand{\CT}{{\cal T}}
\newcommand{\CU}{{\cal U}}
\newcommand{\CV}{{\cal V}}
\newcommand{\CW}{{\cal W}}
\newcommand{\CX}{{\cal X}}
\newcommand{\CY}{{\cal Y}}
\newcommand{\CZ}{{\cal Z}}
% Abbreviate symbols for bold caligraphic letters
\newcommand{\BCa}{{\bfm{\cal a}}}
\newcommand{\BCb}{{\bfm{\cal b}}}
\newcommand{\BCc}{{\bfm{\cal c}}}
\newcommand{\BCd}{{\bfm{\cal d}}}
\newcommand{\BCe}{{\bfm{\cal e}}}
\newcommand{\BCf}{{\bfm{\cal f}}}
\newcommand{\BCg}{{\bfm{\cal g}}}
\newcommand{\BCh}{{\bfm{\cal h}}}
\newcommand{\BCi}{{\bfm{\cal i}}}
\newcommand{\BCj}{{\bfm{\cal j}}}
\newcommand{\BCk}{{\bfm{\cal k}}}
\newcommand{\BCl}{{\bfm{\cal l}}}
\newcommand{\BCm}{{\bfm{\cal m}}}
\newcommand{\BCn}{{\bfm{\cal n}}}
\newcommand{\BCo}{{\bfm{\cal o}}}
\newcommand{\BCp}{{\bfm{\cal p}}}
\newcommand{\BCq}{{\bfm{\cal q}}}
\newcommand{\BCr}{{\bfm{\cal r}}}
\newcommand{\BCs}{{\bfm{\cal s}}}
\newcommand{\BCt}{{\bfm{\cal t}}}
\newcommand{\BCu}{{\bfm{\cal u}}}
\newcommand{\BCv}{{\bfm{\cal v}}}
\newcommand{\BCx}{{\bfm{\cal x}}}
\newcommand{\BCy}{{\bfm{\cal y}}}
\newcommand{\BCz}{{\bfm{\cal z}}}
\newcommand{\BCA}{{\bfm{\cal A}}}
\newcommand{\BCB}{{\bfm{\cal B}}}
\newcommand{\BCC}{{\bfm{\cal C}}}
\newcommand{\BCD}{{\bfm{\cal D}}}
\newcommand{\BCE}{{\bfm{\cal E}}}
\newcommand{\BCF}{{\bfm{\cal F}}}
\newcommand{\BCG}{{\bfm{\cal G}}}
\newcommand{\BCH}{{\bfm{\cal H}}}
\newcommand{\BCI}{{\bfm{\cal I}}}
\newcommand{\BCJ}{{\bfm{\cal J}}}
\newcommand{\BCK}{{\bfm{\cal K}}}
\newcommand{\BCL}{{\bfm{\cal L}}}
\newcommand{\BCM}{{\bfm{\cal M}}}
\newcommand{\BCN}{{\bfm{\cal N}}}
\newcommand{\BCO}{{\bfm{\cal O}}}
\newcommand{\BCP}{{\bfm{\cal P}}}
\newcommand{\BCQ}{{\bfm{\cal Q}}}
\newcommand{\BCR}{{\bfm{\cal R}}}
\newcommand{\BCS}{{\bfm{\cal S}}}
\newcommand{\BCT}{{\bfm{\cal T}}}
\newcommand{\BCU}{{\bfm{\cal U}}}
\newcommand{\BCV}{{\bfm{\cal V}}}
\newcommand{\BCW}{{\bfm{\cal W}}}
\newcommand{\BCX}{{\bfm{\cal X}}}
\newcommand{\BCY}{{\bfm{\cal Y}}}
\newcommand{\BCZ}{{\bfm{\cal Z}}}


\def\ii{{\rm i}}
\def\dd{{\rm d}}
\def\Im{{\it Im}}
\def\Re{{\it Re}}
\def\ca{{\cal A}}
\def\ct{{\cal T}}
\def\Ba{{\bf a}}
\def\Bb{{\bf b}}
\def\Bc{{\bf c}}
\def\Bd{{\bf d}}
\def\Be{{\bf e}}
\def\Bf{{\bf f}}
\def\Bg{{\bf g}}
\def\Bh{{\bf h}}
\def\Bi{{\bf i}}
\def\Bj{{\bf j}}
\def\Bk{{\bf k}}
\def\Bl{{\bf l}}
\def\Bm{{\bf m}}
\def\Bn{{\bf n}}
\def\Bo{{\bf o}}
\def\Bp{{\bf p}}
\def\Bq{{\bf q}}
\def\Br{{\bf r}}
\def\Bs{{\bf s}}
\def\Bt{{\bf t}}
\def\Bu{{\bf u}}
\def\Bv{{\bf v}}
\def\Bw{{\bf w}}
\def\Bx{{\bf x}}
\def\By{{\bf y}}
\def\Bz{{\bf z}}
\def\BA{{\bf A}}
\def\BB{{\bf B}}
\def\BC{{\bf C}}
\def\BD{{\bf D}}
\def\BE{{\bf E}}
\def\BF{{\bf F}}
\def\BG{{\bf G}}
\def\BH{{\bf H}}
\def\BI{{\bf I}}
\def\BJ{{\bf J}}
\def\BK{{\bf K}}
\def\BL{{\bf L}}
\def\BM{{\bf M}}
\def\BN{{\bf N}}
\def\BO{{\bf O}}
\def\BP{{\bf P}}
\def\BQ{{\bf Q}}
\def\BR{{\bf R}}
\def\BS{{\bf S}}
\def\BT{{\bf T}}
\def\BU{{\bf U}}
\def\BV{{\bf V}}
\def\BW{{\bf W}}
\def\BX{{\bf X}}
\def\BY{{\bf Y}}
\def\BZ{{\bf Z}}

\def\half{{\scriptstyle{1\over 2}}}
\newcommand{\eps}{\varepsilon}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\overliner}{\begin{eqnarray}}
\newcommand{\earr}{\end{eqnarray}}
\newcommand{\beqn}{\begin{equation*}}
\newcommand{\eeqn}{\end{equation*}}
\newcommand{\overlinern}{\begin{eqnarray*}}
\newcommand{\earrn}{\end{eqnarray*}}
\newcommand{\prt}{\partial}
\newcommand{\sg}{\sigma}
\newcommand{\fr}{\frac}
\newcommand{\kap}{\varkappa}
%\newcommand{\diag}{\mbox{diag}}
\newcommand{\sign}{\mbox{sign}}
\def\l{\label}

